Sensitivity-driven adaptive sparse stochastic approximations in plasma microinstability analysis

Quantifying uncertainty in predictive simulations for real-world problems is of paramount importance - and far from trivial, mainly due to the large number of stochastic parameters and significant computational requirements. Adaptive sparse grid approximations are an established approach to overcome these challenges. However, standard adaptivity is based on global information, thus properties such as lower intrinsic stochastic dimensionality or anisotropic coupling of the input directions, which are common in practical applications, are not fully exploited. We propose a novel structure-exploiting dimension-adaptive sparse grid approximation methodology using Sobol' decompositions in each subspace to introduce a sensitivity scoring system to drive the adaptive process. By employing local sensitivity information, we explore and exploit the anisotropic coupling of the stochastic inputs as well as the lower intrinsic stochastic dimensionality. The proposed approach is generic, i.e., it can be formulated in terms of arbitrary approximation operators and point sets. In particular, we consider sparse grid interpolation and pseudo-spectral projection constructed on (L)-Leja sequences. The power and usefulness of the proposed method is demonstrated by applying it to the analysis of gyrokinetic microinstabilities in fusion plasmas, one of the key scientific problems in plasma physics and fusion research. In this context, it is shown that a 12D parameter space can be scanned very efficiently, gaining more than an order of magnitude in computational cost over the standard adaptive approach. Moreover, it allows for the uncertainty propagation and sensitivity analysis in higher-dimensional plasma microturbulence problems, which would be almost impossible to tackle with standard screening approaches.

==> sections/05_postproc.tex <==
\section{Postprocessing} \label{sec:postproc}

The pseudo-spectral coefficients for either PSP or interpolation can be used to perform the entire postprocessing in forward UQ.
To this end, in \cite{Su08, Xi10} it was shown that the expectation, standard deviation and total Sobol' indices for variance-based global sensitivity analysis can be computed from the pseudo-spectral coefficients. 

For either interpolation or PSP, let $\{c_{\boldsymbol{p}}\}_{\boldsymbol{p} = \boldsymbol{0}}^{\boldsymbol{P}_{\mathcal{L}, \mathrm{op}}}$ denote the pseudo-spectral coefficients at the end of the adaptive refinement, where $\boldsymbol{P}_{\mathcal{L}, \mathrm{op}}$ is the corresponding total multivariate degree.
The expectation, $\mathbb{E}[\boldsymbol{\mathcal{U}}_{\mathcal{L}, \mathrm{op}}^{(d)}]$, standard deviation, $\sigma[\boldsymbol{\mathcal{U}}_{\mathcal{L}, \mathrm{op}}^{(d)}]$, and total Sobol' index $S_i^T$ in direction $i$ are assessed as:
\begin{align*}
\mathbb{E}[\boldsymbol{\mathcal{U}}_{\mathcal{L}, \mathrm{op}}^{(d)}] = c_{\boldsymbol{0}}  \\ 
\sigma[\boldsymbol{\mathcal{U}}_{\mathcal{L}, \mathrm{op}}^{(d)}] = \sqrt{\sum_{\boldsymbol{p} \neq \boldsymbol{0}} c_{\boldsymbol{p}}^2}  \\
S_i^T = \frac{\sum_{\boldsymbol{k} \in \mathcal{K}_{i, \mathrm{op}}} c_{\boldsymbol{k}}^2}{\sigma^2[\boldsymbol{\mathcal{U}}_{\mathcal{L}, \mathrm{op}}^{(d)}]},
\end{align*}
where $\mathcal{K}_{i, \mathrm{op}} = \{\boldsymbol{0} < \boldsymbol{k} \leq \boldsymbol{P}_{\mathcal{L}, \mathrm{op}}: \boldsymbol{k}_i \neq 0 \}$.
Total Sobol' indices comprise the total contribution of a stochastic input to the resulting variance, i.e., its individual contribution as well as contributions due to interactions with other inputs.
Therefore, the sum of all these total indices is usually greater than $1$, since the interaction contributions are added multiple times.
If this sum is close to $1$, the interactions between the stochastic inputs are negligible, therefore, the underlying stochastic model can be well approximated with a linear (multivariate) function.
For more details on Sobol' indices, we refer to \cite{Su08, Xi10}.
